First look at data from the 13-antenna setup of GRANDProto300 in northwest China

The Giant Radio Array for Neutrino Detection (GRAND) is an envisioned observatory of ultra-high-energy neutrinos, cosmic rays, and gamma rays, with energies above 100 PeV. GRAND targets the radio signals emitted by extensive air showers induced by the interaction of ultra-high-energy particles in the atmosphere, using an array of 200,000 radio antennas split into sub-arrays deployed worldwide. GRANDProto13 (GP13) is a 13-antenna demonstrator array deployed in February 2023 in the Gansu province of China, as a precursor for GRANDProto300, which will validate the detection principle of the GRAND experiment. Its goal is to measure the radio background present at the site, validate the design of the detection units and develop an autonomous radio trigger for air showers. We will describe GP13 and its operation, and show preliminary results on noise monitoring.

==> authors.tex <==
{
 "cells": [
  {
   "cell_type": "code",
   "execution_count": null,
   "id": "01881d37",
   "metadata": {},
   "outputs": [],
   "source": [
    "# File name: authors.ipnyb\n",
    "\n",
    "# Created: 24/06/2023 (Mauricio Bustamante, mbustamante@gmail.com)\n",
    "# Last update: 26/06/2023  (Mauricio Bustamante, mbustamante@gmail.com)\n",
    "\n",
    "# Description:\n",
    "# Script to generate a list of GRAND Collaboration authors in text form, for use in publications.\n",
    "\n",
    "# Input:\n",
    "# A pre-generated, external database file (members.db) that can be queried using SQL."
   ]
  },
  {
   "cell_type": "code",
   "execution_count": 109,
   "id": "b2ed43e9",
   "metadata": {},
   "outputs": [],
   "source": [
    "import sqlite3\n",
    "from pylatexenc.latexencode import unicode_to_latex # To install: pip install pylatexenc \n",
    "import numpy as np\n",
    "\n",
    "# Comment out the call to pylatexenc above if conversion from Unicode to LaTeX is not needed.\n",
    "# In that case, also set convert_unicode_to_latex = False below."
   ]
  },
  {
   "cell_type": "code",
   "execution_count": 47,
   "id": "4e1aa6af",
   "metadata": {},
   "outputs": [],
   "source": [
    "# Open the database, create a cursor to point at it\n",
    "con = sqlite3.connect('members.db')\n",
    "cur = con.cursor()\n",
    "\n",
    "# Select active members only (those that have is_member==1)\n",
    "active_members = cur.execute('SELECT names, surname, names_local, surname_local, institute1_id, institute2_id, \\\n",
    "                      institute3_id, institute4_id, institute5_id FROM grandmember WHERE is_member=1 \\\n",
    "                      ORDER BY surname COLLATE NOCASE ASC').fetchall()\n",
    "# for member in active_members:\n",
    "#     print(member)\n",
    "\n",
    "# Fetch the institutions\n",
    "institutions = cur.execute('SELECT id, name, name_local, address, address_local FROM institute').fetchall()\n",
    "# for inst in institutions:\n",
    "#     print(inst)\n",
    "\n",
    "# Close the database\n",
    "con.close()"
   ]
  },
  {
   "cell_type": "code",
   "execution_count": 128,
   "id": "0a9ae9fd",
   "metadata": {},
   "outputs": [],
   "source": [
    "use_initials = True             # True: use initials for names; False: use full names\n",
    "convert_unicode_to_latex = True # True: convert Unicode characters to LaTex; False: don't (need pylatexenc)"
   ]
  },
  {
   "cell_type": "code",
   "execution_count": 129,
   "id": "70484a75",
   "metadata": {},
   "outputs": [
    {
     "name": "stdout",
     "output_type": "stream",
     "text": [
      "['J.~Alvarez-Muniz$^{1}$,' 'R.~A.~Batista$^{2}$,' 'A.~Benoit-Levy$^{3}$,'\n",
      " 'T.~Bister$^{4, 5}$,' 'J.~Bolmont$^{6}$,' 'M.~Bustamante$^{7}$,'\n",
      " 'D.~Charrier$^{8}$,' 'Y.~Chen$^{9}$,' 'L.~Cheng$^{10}$,'\n",
      " 'S.~Chiche$^{11}$,' 'J.~Colley$^{6}$,' 'P.~Correa$^{6}$,'\n",
      " 'N.~Cucu Laurenciu$^{4}$,' 'Z.~Dai$^{12}$,' 'R.~M.~de Almeida$^{13}$,'\n",
      " 'S.~de Jong$^{4}$,' 'J.~R.~T.~de Mello Neto$^{14}$,'\n",
      " 'K.~D.~de Vries$^{15}$,' 'P.~B.~Denton$^{16}$,' 'V.~Deocoene$^{11}$,'\n",
      " 'K.~Duan$^{9}$,' 'R.~Duan$^{10}$,' 'B.~Duan$^{9}$,'\n",
      " 'R.~Engel$^{17, 18}$,' 'Y.~Fan$^{9}$,' 'K.~Fang$^{19}$,'\n",
      " 'A.~Ferri\\\\`ere$^{20}$,' 'Q.~Gou$^{21}$,' 'J.~Gu$^{10}$,'\n",
      " 'M.~Guelfand$^{6, 11}$,' 'L.~Guelzow$^{17}$,' 'C.~Guepin$^{22, 23}$,'\n",
      " 'J.~Guo$^{9}$,' 'Y.~Guo$^{21}$,' 'V.~Gupta$^{17}$,' 'A.~Haungs$^{17}$,'\n",
      " 'H.~He$^{9}$,' 'E.~Hivon$^{11}$,' 'H.~Hu$^{21}$,' 'X.~Huang$^{9}$,'\n",
      " 'Y.~Huang$^{10}$,' 'T.~Huege$^{24, 17}$,' 'W.~Jiang$^{25}$,'\n",
      " 'R.~Koirala$^{26, 27}$,' 'K.~Kotera$^{28, 11}$,' 'J.~K\\\\\"ohler$^{17}$,'\n",
      " 'B.~L.~Lago$^{29}$,' 'S.~Le Coz$^{6}$,' 'F.~Legrand$^{6}$,'\n",
      " 'J.~Lenain$^{6}$,' 'H.~Li$^{25}$,' 'R.~Li$^{25}$,' 'C.~Liu$^{21}$,'\n",
      " 'R.~Liu$^{26, 27}$,' 'W.~Liu$^{21}$,' 'P.~Ma$^{9}$,' 'F.~Magnard$^{11}$,'\n",
      " 'O.~Martineau-Huynh$^{10, 6, 11}$,' 'A.~Mikhno$^{11}$,'\n",
      " 'P.~Mitra$^{30}$,' \"M.~Mostaf\\\\'a$^{31, 32}$,\" 'F.~Mottez$^{33}$,'\n",
      " 'J.~Mouette$^{11}$,' 'K.~Murase$^{31, 32}$,' 'V.~Niess$^{34}$,'\n",
      " 'S.~Ogio$^{35}$,' 'F.~Oikonomou$^{36}$,' 'Z.~Ou$^{37}$,'\n",
      " 'T.~Pierog$^{17}$,' 'L.~W.~Piotrowski$^{30}$,' 'P.~Poisvert$^{6}$,'\n",
      " 'S.~Prunet$^{38}$,' 'X.~Qian$^{39}$,' 'O.~M.~Ramirez$^{40}$,'\n",
      " 'M.~Roth$^{17}$,' 'T.~Sako$^{35}$,' 'H.~Schoorlemmer$^{4, 5}$,'\n",
      " 'F.~Schussler$^{20}$,' 'B.~Steeman$^{4}$,'\n",
      " \"D.~Sz\\\\'alas-Motesiczky$^{4}$,\" \"S.~S{\\\\l}awi\\\\'nski$^{30}$,\"\n",
      " 'A.~Timmermans$^{15, 4}$,' 'C.~Timmermans$^{4, 5}$,' 'M.~Tueros$^{41}$,'\n",
      " 'S.~Wang$^{9}$,' 'X.~Wang$^{26, 27}$,' 'X.~Wang$^{25}$,'\n",
      " 'X.~Wang$^{39}$,' 'R.~Wang$^{25}$,' 'C.~Watanabe$^{14}$,' 'D.~Wei$^{9}$,'\n",
      " 'F.~Wei$^{25}$,' 'X.~Wu$^{10, 42}$,' 'X.~Wu$^{43}$,' 'X.~Xu$^{25}$,'\n",
      " 'X.~Xu$^{9}$,' 'L.~Yang$^{37}$,' 'X.~Yang$^{9}$,' 'Q.~Yuan$^{9}$,'\n",
      " 'P.~Zarka$^{44}$,' 'H.~Zeng$^{9}$,' 'C.~Zhang$^{45, 46, 17}$,'\n",
      " 'J.~Zhang$^{10}$,' 'K.~Zhang$^{9}$,' 'P.~Zhang$^{25}$,'\n",
      " 'S.~Zhang$^{43}$,' 'H.~Zhang$^{25}$,' 'H.~Zhou$^{47}$']\n"
     ]
    }
   ],
   "source": [
    "# Export author names and institutions in this format:\n",
    "# Name Surname^{m,n}\n",
    "# ${^m}$Institution1\n",
    "# ${^n}$Institution2\n",
    "\n",
    "# First create the author entries\n",
    "member_list = np.array([])\n",
    "# selected_institutions stores stores the database IDs and print IDs of the institutions that have already appeared\n",
    "selected_institutions = np.array([]) \n",
    "dict_selected_institutions = {}\n",
    "inst_index_print = 1\n",
    "num_active_members = len(active_members)\n",
    "for i, member in enumerate(active_members):\n",
    "#     print(member)\n",
    "    # For each member, create a text string containing the name and affiliation call\n",
    "    names, surname, names_local, surname_local, institute1_id, institute2_id, institute3_id, institute4_id, \\\n",
    "        institute5_id = member\n",
    "    if convert_unicode_to_latex:\n",
    "        names = unicode_to_latex(names)\n",
    "        surname = unicode_to_latex(surname)\n",
    "        names_local = unicode_to_latex(unicode_to_latex)\n",
    "        surname_local = unicode_to_latex(surname_local)\n",
    "    if use_initials:\n",
    "        names = ''.join([x[0].upper()+r'.~' for x in names.split(' ')])\n",
    "        member_string = names+surname # Name Surname    \n",
    "    else:\n",
    "        member_string = names+' '+surname # Name Surname\n",
    "    member_string += r'$^{'\n",
    "    flag_first_inst = True\n",
    "    for inst_index in [institute1_id, institute2_id, institute3_id, institute4_id, institute5_id]:\n",
    "        if inst_index is not None:\n",
    "            if not inst_index in np.array(list(dict_selected_institutions.keys())):\n",
    "                dict_selected_institutions[inst_index] = inst_index_print\n",
    "                inst_index_print += 1\n",
    "            if not flag_first_inst: member_string += r', '\n",
    "            member_string += str(dict_selected_institutions[inst_index]) #str(inst)\n",
    "            flag_first_inst = False\n",
    "    member_string += r'}$'\n",
    "    if (i != num_active_members-1):\n",
    "        member_string += ','\n",
    "    member_list = np.append(member_list, member_string)\n",
    "#     print(member_string)\n",
    "print(member_list)"
   ]
  },
  {
   "cell_type": "code",
   "execution_count": 131,
   "id": "f42893c6",
   "metadata": {},
   "outputs": [
    {
     "name": "stdout",
     "output_type": "stream",
     "text": [
      "['$^{1}$Departamento de Fisica de Particulas \\\\& Instituto Galego de Fisica de Altas Enerxias, Universidad de Santiago de Compostela, 15782 Santiago de Compostela, Spain'\n",
      " \"$^{2}$Instituto de F{\\\\'\\\\i}sica Te\\\\'orica, Universidad Aut\\\\'onoma de Madrid - CSIC, 28049 Madrid, Spain\"\n",
      " \"$^{3}$CEA List, Universit\\\\'e Paris-Saclay,  F-91120 Palaiseau, France\"\n",
      " '$^{4}$Institute for Mathematics, Astrophysics and Particle Physics, Radboud Universiteit, Nijmegen, Netherlands'\n",
      " '$^{5}$Nationaal Instituut voor Kernfysica en Hoge Energie Fysica, '\n",
      " '$^{6}$Universite Paris Diderot, Sorbonne Paris Cite, CNRS Laboratoire de Physique Nucleaire et de Hautes Energies, 4 place Jussieu F-75252, Paris Cedex 5, France'\n",
      " '$^{7}$Niels Bohr International Academy, Niels Bohr Institute, University of Copenhagen, 2100 Copenhagen, Denmark'\n",
      " '$^{8}$SUBATECH, Institut Mines-Telecom Atlantique, CNRS/IN2P3, Universite de Nantes, Nantes, France'\n",
      " '$^{9}$Key Laboratory of Dark Matter and Space Astronomy, Purple Mountain Observatory, Chinese Academy of Sciences, 210023 Nanjing, Jiangsu, China'\n",
      " '$^{10}$National Astronomical Observatories, Chinese Academy of Sciences, Beijing 100101, China'\n",
      " \"$^{11}$ Institut d'Astrophysique de Paris, CNRS  UMR 7095, Sorbonne Universite, 98 bis bd Arago 75014, Paris, France\"\n",
      " '$^{12}$University of Science and Technology of China, 230026 Hefei  Anhui, China'\n",
      " '$^{13}$Universidade Federal Fluminense, EEIMVR Volta Redonda RJ, Brazil'\n",
      " '$^{14}$Instituto de Fisica, Universidade Federal do Rio de Janeiro, '\n",
      " '$^{15}$IIHE/ELEM, Vrije Universiteit Brussel, Pleinlaan 2, 1050 Brussels, Belgium'\n",
      " '$^{16}$High Energy Theory Group, Physics Department Brookhaven National Laboratory, Upton, NY 11973, USA'\n",
      " '$^{17}$Institute for Astroparticle Physics, Karlsruhe Institute of Technology, D-76021 Karlsruhe, Germany'\n",
      " '$^{18}$Institute of Experimental Particle Physics, Karlsruhe Institute of Technology, D-76021 Karlsruhe, Germany'\n",
      " '$^{19}$Wisconsin IceCube Particle Astrophysics Center and Deptartment of Physics, University of Wisconsin-Madison, Madison, WI 53703, USA'\n",
      " '$^{20}$IRFU, CEA Universite Paris-Saclay, F-91191 Gif-sur-Yvette, France'\n",
      " '$^{21}$Institute of High Energy Physics, Chinese Academy of Sciences, 19B YuquanLu, Beijing 100049, China'\n",
      " '$^{22}$Department of Astronomy, University of Maryland, College Park, MD 20742-2421, USA'\n",
      " '$^{23}$Joint Space-Science Institute, College Park, MD 20742-2421, USA'\n",
      " '$^{24}$Astrophysical Institute, Vrije Universiteit Brussel, Pleinlaan 2, 1050 Brussels, Belgium'\n",
      " '$^{25}$Key Laboratory of Antennas and Microwave Technology, Xidian University, Xi{\\\\textquoteright}an 710071, China'\n",
      " '$^{26}$School of Astronomy and Space Science, Nanjing University, Xianlin Road 163, Nanjing 210023, China'\n",
      " '$^{27}$Key laboratory of Modern Astronomy and Astrophysics, Nanjing University, Ministry of Education, Nanjing 210023, China'\n",
      " '$^{28}$Vrije Universiteit Brussel, Pleinlaan 2, B-1050 Brussels, Belgium'\n",
      " \"$^{29}$Centro Federal de Educa\\\\c{c}\\\\~ao Tecnol\\\\'ogica Celso Suckow da Fonseca, Nova Friburgo, Brazil\"\n",
      " '$^{30}$Faculty of Physics, University of Warsaw, Pasteura 5, 02-093 Warsaw, Poland'\n",
      " '$^{31}$Department of Astronomy \\\\& Astrophysics, Pennsylvania State University, University Park, PA 16802, USA'\n",
      " '$^{32}$Center for Multimessenger Astrophysics, Pennsylvania State University, University Park, PA 16802, USA'\n",
      " '$^{33}$LUTH, Obs. de Paris CNRS Universite Paris Diderot, PSL Research University, 5 place Jules Janssen 92190, Meudon, France'\n",
      " \"$^{34}$CNRS/IN2P3 LPC, Universit\\\\'e Clermont Auvergne, F-63000 Clermont-Ferrand, France\"\n",
      " '$^{35}$Institute for Cosmic Ray Research, University of Tokyo, 5 Chome-1-5 Kashiwanoha, Kashiwa, Chiba 277-0882, Japan'\n",
      " '$^{36}$Institutt for fysikk, NTNU, Trondheim, Norway'\n",
      " '$^{37}$School of Physics and Astronomy, Sun Yat-sen University, Zhuhai 519082, China'\n",
      " \"$^{38}$Laboratoire Lagrange, Observatoire de la C\\\\^ote d{\\\\textquoteright}Azur, Universite C\\\\^ote d'Azur, CNRS, Parc Valrose 06104, Nice Cedex 2, France\"\n",
      " '$^{39}$Department of Mechanical and Electrical Engineering, Shandong Management University,  Jinan 250357, China'\n",
      " '$^{40}$Gravitation Astroparticle Physics Amsterdam, Univesity of Amsterdam, Science Park 904, 1098 XH Amsterdam, Netherlands'\n",
      " '$^{41}$Instituto de Fisica La Plata, CONICET  Boulevard 120 y 63 (1900)  La Plata'\n",
      " '$^{42}$Shanghai Astronomical Observatory, Chinese Academy of Sciences, 80 Nandan Road, Shanghai 200030, China'\n",
      " '$^{43}$Purple Mountain Observatory, Chinese Academy of Sciences, Nanjing 210023, China'\n",
      " '$^{44}$LESIA, Observatoire de Paris, CNRS, PSL/SU/UPD/SPC, Place J. Janssen 92195, Meudon, France'\n",
      " '$^{45}$Kavli Institute for Astronomy and Astrophysics, Peking University, Beijing 100871, China'\n",
      " '$^{46}$Department of Astronomy, School of Physics, Peking University, Beijing 100871, China'\n",
      " '$^{47}$Tsung-Dao Lee Institute \\\\& School of Physics and Astronomy, Shanghai Jiao Tong University, 200240 Shanghai, China']\n"
     ]
    }
   ],
   "source": [
    "# Now create the institution entries\n",
    "institutions = np.array(institutions)\n",
    "institution_list = np.array([])\n",
    "# print(list(dict_selected_institutions.keys()))\n",
    "for inst_index in list(dict_selected_institutions.keys()):\n",
    "    inst_index_print = dict_selected_institutions[inst_index]\n",
    "    inst = institutions[institutions[:,0] == str(inst_index), :][0]\n",
    "#     print(inst)\n",
    "    name = inst[1]\n",
    "    address = inst[3]\n",
    "    if convert_unicode_to_latex:\n",
    "        name = unicode_to_latex(name)\n",
    "        address = unicode_to_latex(address)\n",
    "    inst_string = r'$^{'+str(inst_index_print) + r'}$' + name + ', ' + address\n",
    "    institution_list = np.append(institution_list, inst_string)\n",
    "print(institution_list)"
   ]
  },
  {
   "cell_type": "code",
   "execution_count": 136,
   "id": "b8e6b3df",
   "metadata": {},
   "outputs": [],
   "source": [
    "# Now export this to a file\n",
    "filename = 'authors.tex'\n",
    "# Save authors\n",
    "np.savetxt(filename, member_list, fmt='%s')\n",
    "# Save institutions\n",
    "with open(filename, 'a') as f:\n",
    "    np.savetxt(f, ['\\\\newline'], fmt='%s')\n",
    "    np.savetxt(f, institution_list, fmt='%s')"
   ]
  },
  {
   "cell_type": "code",
   "execution_count": null,
   "id": "4f7b926c",
   "metadata": {},
   "outputs": [],
   "source": []
  }
 ],
 "metadata": {
  "kernelspec": {
   "display_name": "Python 3",
   "language": "python",
   "name": "python3"
  },
  "language_info": {
   "codemirror_mode": {
    "name": "ipython",
    "version": 3
   },
   "file_extension": ".py",
   "mimetype": "text/x-python",
   "name": "python",
   "nbconvert_exporter": "python",
   "pygments_lexer": "ipython3",
   "version": "3.7.7"
  }
 },
 "nbformat": 4,
 "nbformat_minor": 5
}
